Parallel Batch-Dynamic Algorithms for $k$-Core Decomposition and Related Graph Problems

Maintaining a $k$-core decomposition quickly in a dynamic graph has important applications in network analysis. The main challenge for designing efficient exact algorithms is that a single update to the graph can cause significant global changes. Our paper focuses on \emph{approximation} algorithms with small approximation factors that are much more efficient than what exact algorithms can obtain. We present the first parallel, batch-dynamic algorithm for approximate $k$-core decomposition that is efficient in both theory and practice. Our algorithm is based on our novel parallel level data structure, inspired by the sequential level data structures of Bhattacharya et al [STOC '15] and Henzinger et al [2020]. Given a graph with $n$ vertices and a batch of updates $\mathcal{B}$, our algorithm provably maintains a $(2 + \varepsilon)$-approximation of the coreness values of all vertices (for any constant $\varepsilon > 0$) in $O(|\mathcal{B}|\log^2 n)$ amortized work and $O(\log^2 n \log\log n)$ depth (parallel time) with high probability. As a by-product, our $k$-core decomposition algorithm also gives a batch-dynamic algorithm for maintaining an $O(\alpha)$ out-degree orientation, where $\alpha$ is the current arboricity of the graph. We demonstrate the usefulness of our low out-degree orientation algorithm by presenting a new framework to formally study batch-dynamic algorithms in bounded-arboricity graphs. Our framework obtains new provably-efficient parallel batch-dynamic algorithms for maximal matching, clique counting, and vertex coloring. We implemented and experimentally evaluated our $k$-core decomposition algorithm on a 30-core machine with two-way hyper-threading on $11$ graphs of varying densities and sizes. [...]

==> data-structures.tex <==
\subsection{Data Structure Implementations}\label{sec:data-structure-impl}


Due to  space constraints, we only specify the data structures used
to obtain our randomized (high probability) bounds. We implement
these data structures in our experiments. Our data structures presented here
result in $O(n\log^2 m + m)$ space usage. However, we present two additional
sets of data
structures in
\ificml
the full paper:
\fi
\iflong
\cref{app:data-structure-impl}:
\fi
one that achieves $O(m)$ space with an $O(\log^2 m)$ factor increase in
depth and another that results in a \emph{deterministic} PLDS.

Our data structure uses parallel hash tables, which support $x$
concurrent insertions, deletions, or finds in $O(x)$ amortized work
and $O(\log^*x)$ depth \whp~\cite{Gil91a}.  We use
dynamic arrays, which support adding or deleting $x$ elements from the
end in $O(x)$ amortized work and $O(1)$ depth.

We first assign each vertex a unique ID in $[n]$.
We also maintain an array $\greater$ of size $n$ keyed by vertex ID
that returns a parallel
hash table containing neighbors of $v$ on levels $\geq
\level(v)$.
For each vertex $v$, we maintain a dynamic array $\tbl_v$ keyed by
indices $i \in [0, \level(v) - 1]$.
The $i$'th entry of the array contains a pointer to a parallel hash
table containing the neighbors of $v$ in level $i$.
Appropriate
pointers exist that allow $O(1)$ work to access elements
in structures. Furthermore, we maintain a hash table which contains
pointers to vertices $v$ where $\dl(v) \neq \level(v)$, partitioned by their levels.  This allows us to quickly
determine which vertices to move up (in~\cref{alg:insert}) or move
down (in~\cref{alg:delete}).











==> error-table.tex <==
\begin{table*}[htbp]
\caption{Average and maximum errors of PLDSOpt,
PLDS, and ApproxKCore on insertion-only and
deletion-only batches of size $10^6$. Insertion-only batches
errors are shown on the left 
and deletion-only batches are shown on the right.
* indicates that the error was obtained via sampling
the error probability with $1/10$ probability.
T.O. indicates that the program timed out at 3 hours (even
when performing the sampling with $1/10$ probability).} \label{table:error-exp-4}
\begin{center}
\footnotesize
\begin{tabular}[!t]{|l|r|r|r|r|r|r|}
\toprule
{Graph Dataset} & \shortstack{PLDSOpt\\ Avg.} & \shortstack{PLDSOpt\\ Max}& \shortstack{PLDS\\ Avg.}& \shortstack{PLDS\\ Max} &
\shortstack{Approx\\ KCore\\ Avg.}  & \shortstack{Approx \\ KCore\\ Max} \\
\midrule
{\emph{ dblp  }  }           &   1.9345       &3  & 2.635 & 4 & 1.15 & 3.875\\
{\emph{ brain        }  }        &  1.834       &3  & 3.363& 4.193 & 1.315 & 4.305 \\
{\emph{ wiki  }  } &1.590      &  3 & 1.780 & 4.172 & 1.010 & 3\\
{\emph{ youtube }  }          & 1.359         &3 &  1.593 & 4  & 1.1283 & 3.75\\
{\emph{ stackoverflow }  }    & 1.826      &3 &  2.272 & 4.067 &  1.048 & 3.875 \\
{\emph{ livejournal  }  }    		 &   1.660   & 3  &  2.321 & 4.175 &4.175 & 1.165\\
{\emph{ orkut        }  }    &    1.926   & 3  & 3.115 & 4.175 & 1.204 & 4.2\\
{\emph{ ctr     }  }     &   1.601     & 3   & 1.683 & 3  & 1.374 & 3 \\
{\emph{ usa        }  }     &   1.826     & 3  & 1.683 & 3  & 1.379 & 3 \\
{\emph{ twitter      }  }    	        &2.118* & 3*  & T.O. & T.O. & T.O. & T.O. \\
{\emph{ friendster}}         &1.851* & 3*  &  T.O. & T.O. & T.O. & T.O. \\
\hline
\end{tabular}
\quad
\begin{tabular}[!t]{|l|r|r|r|r|r|r|}
\toprule
{Graph Dataset} & \shortstack{PLDSOpt\\ Avg.} & \shortstack{PLDSOpt\\ Max}& \shortstack{PLDS\\ Avg.}& \shortstack{PLDS\\ Max} &
\shortstack{Approx\\ KCore\\ Avg.}  & \shortstack{Approx\\ KCore\\ Max} \\
\midrule
{\emph{ dblp  }  }       & 1.187  &  6 & 1.507 & 2 &1.236 & 3.0\\
{\emph{ brain        }  }        &1.575 & 6 & 1.943& 4.186&1.315 & 5.0 \\
{\emph{ wiki  }  } &1.423 & 4 &1.494 & 4 &1.013 & 3.875\\
{\emph{ youtube }  }          &1.268 & 4 &1.317 & 4 &1.137 & 3.706\\
{\emph{ stackoverflow }  }    &1.630 & 6 &1.792 & 4.172 &1.045 & 3.908\\
{\emph{ livejournal  }  }    		 &1.613 & 6 &1.704 & 4.14&1.167 & 3.984\\
{\emph{ orkut        }  }    &1.681 & 6 &1.913 & 4.175&1.205 & 4.2\\
{\emph{ ctr     }  }     &1.243 & 3   &1.257 & 3 &1.524 & 3.0\\
{\emph{ usa        }  }     &1.253 & 3 &1.278 & 3  &1.522 & 3.0\\
{\emph{ twitter      }  }    	 &1.893* & 4*     &  T.O. & T.O. & T.O. & T.O.\\
{\emph{ friendster}}     &1.685* & 3* & T.O. & T.O. & T.O. & T.O. \\
\hline
\end{tabular}
\end{center}
\end{table*}




==> implementation.tex <==
\section{$k$-Core Decomposition Experiment Details}\label{sec:exp-implementation}



==> overview.tex <==
\section{Overview of Materials Included}

In these supplementary materials, we include the following items:

\begin{itemize}
    \item A zip file containing the complete anonymized code we used to test our
    experiments. The same version of our code can be found at this URL containing an anonymized Github repository:
    \href{https://anonymous.4open.science/r/e15465a3-efef-4f8e-99cd-9177822220f8/}{webpage link to our code}.
    \item Complete proofs to all of our theorems presented in the Main Paper.
    Namely, the following theorems are proven:
    \begin{itemize}
        \item Theorem 1.1 in~\cref{sec:static-k-core}
        \item Theorem 1.2 at~\cref{thm:batch-dynamic}
        \item Lemma 3.2 at~\cref{lem:move-up}
        \item Lemma 3.3 at~\cref{lem:smaller-level}
        \item Lemma 3.4 at~\cref{cor:depth}
        \item Lemma 3.6 in~\cref{sec:coreness}
    \end{itemize}
    \item We include on and include the proofs for additional results including:
    \begin{itemize}
        \item Additional deterministic and space-efficient data structure
        implementations~\cref{sec:data-structure-impl}.
        \item How to handle batches of vertex insertions and
        deletions~\cref{sec:vertex-ins-del}.
        \item A $(8 + \delta)\alpha$-out-degree orientation
        (\cref{cor:low-outdegree}) and $(8 +
        \delta)$-approximate densest subgraph (\cref{cor:densest-subgraph}).
    \end{itemize}
    \item Complete experimental analysis of deletions tested on the same graphs
    and using the same experimental methods as Section 5 of our Main Paper
    (\cref{sec:exp-delete}).
\end{itemize}

